Fully Convolutional Mesh Autoencoder using Efficient Spatially Varying Kernels

Learning latent representations of registered meshes is useful for many 3D tasks. Techniques have recently shifted to neural mesh autoencoders. Although they demonstrate higher precision than traditional methods, they remain unable to capture fine-grained deformations. Furthermore, these methods can only be applied to a template-specific surface mesh, and is not applicable to more general meshes, like tetrahedrons and non-manifold meshes. While more general graph convolution methods can be employed, they lack performance in reconstruction precision and require higher memory usage. In this paper, we propose a non-template-specific fully convolutional mesh autoencoder for arbitrary registered mesh data. It is enabled by our novel convolution and (un)pooling operators learned with globally shared weights and locally varying coefficients which can efficiently capture the spatially varying contents presented by irregular mesh connections. Our model outperforms state-of-the-art methods on reconstruction accuracy. In addition, the latent codes of our network are fully localized thanks to the fully convolutional structure, and thus have much higher interpolation capability than many traditional 3D mesh generation models.

==> experiment_sections/Interpolation.tex <==
\subsection{Localized Interpolation}
As an additional advantage, the latent codes of our network are localized. We demonstrate this on hand meshes in Figure~\ref{fig:interpolation}. The latent vertices are the tips of the five fingers and the wrist. For interpolation, we first inferred the latent codes from a source mesh and a target mesh, then we linearly interpolated the latent code on each individual latent vertex separately as shown in Figure \ref{fig:interpolation}. With only two input hand models, we can obtain many more gestures by interpolating a subset of latent vertices instead of the entire code.
%\vspace{-3mm}
\begin{figure}
    \includegraphics[width=\linewidth]{fig/hand_interpolation.jpg}
    \caption{Interpolation from source to target using global or local latent codes.}
    \label{fig:interpolation}
\end{figure}
%\vspace{-5mm}

% If we replace our graph sampling scheme with quadric mesh simplification as in \cite{Ranjan_2018_ECCV,bouritsas2019neural}, one cannot achieve the same quality of interpolation. To visualize this, in addition to Figure~\ref{fig:receptive_field}, we mixed the latent codes from two meshes in DFAUST and show the decoded results using our method and the quadric method in Figure~\ref{fig:latent_code_comparison}. In this example, we used six supporting vertices in part 1(red) and on in part 2(green) and decoded the mixture of latent codes to a 3D mesh. Using our method, the output mesh preserves the shape of part 1 and has the right arm drops down as in Part 2. While using the quadratic sampling method, the green latent code impacted the whole body and led to big distortions.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\linewidth]{fig/latent_code_comparison.png}
%     \caption{Comparison of mixing latent codes of two 3D meshes.}
%     \label{fig:latent_code_comparison}
% \end{figure}








==> experiment_sections/N_or_non_manifold.tex <==
\subsection{N-D Manifold and Non-Manifold Meshes}
Different from \cite{Ranjan_2018_ECCV,bouritsas2019neural,hanocka2019meshcnn}, which are limited to 2-D manifold meshes, our method can be applied to N-D manifold or even non-manifold meshes. 

We first demonstrate 3-D manifold cases using 3D tetrahedron meshes (tet mesh). Tet meshes are commonly used for physical simulation~\cite{Vega}. We used a dataset containing 10k deformed tet meshes of an Asian dragon\footnote{The original mesh was created by Stanford Computer Graphics Laboratory, available at \url{http://graphics.stanford.edu/data}, and then simulated using Vega~\cite{Vega}.}, and trained an auto-encoder using 7k for training, 1.3k for validation and 562 for testing. The dragon has 959 vertices and lies in a bounding box of roughly 20$\times$20$\times$20 cm. The auto-encoder has five down-sampling residual blocks and five up-sampling residual blocks. $s=2, r=2, M=37$ for all blocks. Its bottle neck has two vertices, 16 latent codes per vertex. After 400 epochs of training, the error converged to 0.2 mm. Figure ~\ref{fig:asianDragon} shows the cases of input tet meshes, output tet meshes, and the fine surface mesh driven by the output tet meshes. 



To demonstrate our network on non-manifold data, we show our network on a 3D tree model\footnote{The model is from \url{https://www.turbosquid.com/3d-models/cherry-blossom-tree-3d-1189864}}. The tree model has 328 disconnected components. To connect all the components, we added an edge between each pair of close components. We constructed a dataset of 10 sequence of this tree's animation simulated by Vega using random forces, 1000 frames for each clip, and used 2 clips for testing, 2 clips for validation and the rest for training.
The auto-encoder had four down-sampling residual blocks to compress the original 20k vertices into 149 vertices, 8 latent codes per vertex and four up-sampling residual blocks. $s=2, r=2, M=27$ for each block. After 36 epochs of training, the reconstruction error dropped to 4.1 cm. Figure~\ref{fig:tree} shows the ground truth meshes rendered by the receptive field and the output mesh rendered by per vertex error. 




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\begin{table}[]
%\begin{tabular}{|l|l|l|l|l|}
%\hline
%                       & \multicolumn{1}{c|}{Position} & \multicolumn{1}{c|}{Laplace} & \multicolumn{1}{c|}{Zero Weight Coeff}  & \multicolumn{1}{c|}{Inference Time} \\ \hline
%without regularization & 0.017                         & 0.034                        & 0.6\%   & 0.012 (TitanXP)                     \\ \hline
%with regularization    & 0.022                         & 0.044                        & 34.8\%  & 0.016 (TitanXP)                     \\ \hline
%\end{tabular}
%\caption{Results of Volumetric Meshes.}
%\label{tab:results_tet}
%\end{table}


%\begin{table}[]
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
%\hline
%                          & \multicolumn{5}{l|}{Encoder}   & \multicolumn{5}{l|}{Decoder} \\ \hline
%Layer                     & 1    & 2    & 3    & 4   & 5   & 6   & 7   & 8   & 9   & 10   \\ \hline
%Out Vertices              & 199  & 49   & 16   & 5   & 2   & 5   & 16  & 49  & 199 & 1985 \\ \hline
%Channel                   & 16   & 32   & 64   & 128 & 16  & 128 & 64  & 32  & 16  & 3    \\ \hline
%zero weight coeff & 61\% & 32\% & 26\% & 5\% & 2\% & 1\% & 3\% & 5\% & 8\% & 14\% \\ \hline
%\end{tabular}
%\caption{Network Architecture for Volumetric Meshes Experiment. }
%\label{tab:network_tet}
%\end{table}

==> experiment_sections/high_resolution_mesh.tex <==
\subsection{High Resolution Mesh}
Real-world 3D data can have much higher resolution than DFAUST. Here we tested our network on two high-resolution body datasets. 
The first dataset contains fully aligned hand meshes reconstructed from performance captures of two people with roughly 200 seconds of 90 poses per person. The mesh has 57k vertices and 115k facets. We randomly picked 39 one-second clips for testing, 39 one-second clips for validation, and used the rest for training, resulting in 9376 meshes for training and 1170 for testing.  Each vertex is given both the 3D coordinate and RGB color as input. Our auto-encoder network has nine down-sampling residual blocks and nine up-sampling residual blocks with $s=2$, $r=2$ and $M=17$ for all blocks. The latent space has 6 vertices with 64 dimensions per vertex, resulting in a compression rate of 0.11\%. The middle 6 vertices were manually selected to be at the fingertips and wrist. We trained the network with point to point L1 loss, L1 laplacian loss and L1 RGB loss. After 205 epochs of training, the mean point to point euclidean distance error dropped to 1.06 mm and the mean L1 RGB error to 0.036 (range 0 to 1).

%\vspace{-5mm}
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{fig/high_res.png}
    \caption{Result on high resolution mesh.}
    \label{fig:hrbody}
\end{figure}
%\vspace{-5mm}
The second dataset contains 24,628 fully aligned body meshes reconstructed from a performance capture of one person conducting different poses. The resolution for each mesh is 154k vertices and 308k triangles. We randomly chose $2,463$ for validation and used the rest for training. Each vertex has 3D coordinates as the feature to reconstruct. Our auto-encoder has $6$ down-sampling residual blocks and $6$ up-sampling residual blocks, with $s=2$,$r=2$ and $M=17$ for all blocks. The latent space has 18 vertices and 64 dimensions per vertex, resulting in a compression rate of 0.75\%. We additionally used L1 laplacian loss for training. After training $100$ epochs, the mean point to point euclidean distance error dropped to $2.15$ mm for training and $3.01$ mm for validation. From Figure \ref{fig:hrbody} we can see that the output mesh is quite detailed. Compared with the groundtruth, which is more noisy, the network output is relatively smoothed. Interestingly, from the middle two images, we can see that the network learned to reconstruct the vein in the inner side of the arm from the originally noisy surface. 



==> experiment_sections/network_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\subsection{Comparison of Network Architectures}
\label{sec:comparison_of_Architectures}

We compare our method with that of Neural3DMM~\cite{bouritsas2019neural} which is the current state-of-the-art auto-encoder for registered 3D meshes, as well as  MeshCNN~\cite{hanocka2019meshcnn}. % which is a recent work for 3D mesh convolution.

We choose to work with the D-FAUST human body dataset as it captures both high-frequency variance in poses and low-frequency variance in local details. The D-FAUST dataset contains 140 sequences of registered human body meshes. We use 103 sequences (32933 meshes in total) for training, 13 sequences (4023 meshes) for validation and 13 sequences (4264 meshes) for testing. 



We trained our network with 200 epochs, batch size=16, learning rate=0.0001, learning rate decay=0.9 every epoch, using Geforce 1080Ti, cuda 10.0 and pytorch 1.0. For Neural3DMM, we set its latent space dimension to be 63 to match our bottle neck size and trained it with 300 epochs using the exact settings described in its paper. As reported in Table~\ref{tab:network_comparison}, our network achieves over 30\% and 40\% lower errors for the testing and training set respectively with less training epochs and a similar number of parameters. Moreover, Neural3DMM compresses the input mesh into a fully connected bottleneck, while ours is fully convolutional and directly compresses the mesh to 7 vertices, 9 channels per vertex. A visual comparison between the two methods can be found in Figure~\ref{fig:DFAUST_result}. %Our results have smaller areas for large errors and very low errors in the facial area, which implies our method can better preserve both the high or low-frequency information in the signal. 

%For MeshCNN~\cite{hanocka2019meshcnn}, we found that it could not downsample the D-FAUST mesh to less than 1k vertices because of the boundary limitations in its algorithm. 
For MeshCNN~\cite{hanocka2019meshcnn}, we found that it was infeasible to train a model on the full resolution D-FAUST dataset due to memory constraints. Thus, we down-sampled all meshes to 750 vertices, which is the same size they use in their experiments. Because ~\cite{hanocka2019meshcnn} performs convolution on the edges, we use each edge's two endpoints as the input feature we attempt to reconstruct. We set the input size to 3000 edges and have a bottleneck layer of 150 edges. The number layers and channels is the same as in ~\cite{hanocka2019meshcnn}. We train for 200 epochs. 
%\vspace{-5mm}
\begin{figure}
    \includegraphics[width=\linewidth]{fig/reconstruction_results.jpg}
    \caption{Reconstruction results for different meshes and compression ratios.}
    \label{fig:DFAUST_result}
\end{figure}












%\begin{table}[]
%\begin{tabular}{|l|l|l|l|l|l|l|}
%\hline
%          & \multicolumn{2}{l|}{P2P Error} & \multicolumn{2}{l|}{+RigidTrans} & \multirow{2}{*}{Param} & \multirow{2}{*}{Infer} \\ \cline{1-5}
%          & Train          & Test          & Train           & Test           &                        &                        \\ \hline
%Ours      & 3.71           & 5.18          & 9.14(198)       & 9.64           &                        &                        \\ \hline
%Spiral 64 & 6.42           & 7.39          & 11.40           & 11.94          & 676k                   & 0.0049                 \\ \hline
%Spiral 66 & 6.11           & 7.14          &                 &                &                        &                        \\ \hline
%MeshCNN   &                &               &                 &                &                        &                        \\ \hline
%\end{tabular}
%\caption{DFAUST Result and Comparison with SOTA. 290 Epoch. }
%\end{table}








%GAT, MoNet, Spiral and Spectrum CNN cannot be defined as deconvolution with stride.

%According to the report in GAT, it outperfroms MoNet which is its general form, so we don't perform extra experience for MoNet.
%For GAT, we use multi-head-number K=8 and average the head at each layer in order to keep the output feature dimension the same as the rest experiments.
